First-principles derivation of elastic interaction between Jahn-Teller centers in crystals via lattice Green's functions

Jahn-Teller (JT) systems with strong and intermediate vibronic coupling are described in terms of local JT active vibrational modes. In JT crystals, the elastic interaction of these modes at different JT centers plays a crucial role, for instance, in determining critical temperature of structural phase transitions. Despite their importance, the parameters of elastic interaction between JT centers have not been accessed yet by first-principles calculations. In this paper, we develop an effective Hamiltonian methodology for the thorough description of the elastic interactions in cooperative Jahn-Teller problems, which treats the interactions with both phonons and uniform strains. All the microscopic parameters, such as lattice Green's functions, elastic modulus, can be obtained or calculated based on first-principles the calculation. The method has been applied to a series of 5d1 double perovskites. Such effective Hamiltonian methodology can be, in general, used to investigate the APES of any type of the local distortions, such as impurities, defects, etc.

==> EccsUS_summary_Latex_5_onlytwo <==
\begin{table}  
\caption{\label{tab:ECCsUS_summary_all_onlytwo} 
$\Xi$ matrix contributed from uniform starin for the four JT active centers in unconvention unit cell. JTC1, JTC2, JTC3 are the label for the JT active centers, as defined in Table. \ref{Table:coordinates_SAJTmodes_Oct}. From the left to right, and from the top to bottom, the matrix elements correspond to JTD\_2, JTD\_3, JTD\_4, JTD\_5 and JTD\_6, respectively. The unit is $bohr^2/Ry$.} 
\resizebox{0.5\textwidth}{!}{  
\begin{tabular}{|c|c|c|}\hline  
& (0,0,0) (JTC1,JTC1) & (0,0,0) (JTC1,JTC2)  \\ \hline  
NaOs & $ \left( \begin{array}{ccccc}0.267 &0.000 &0.000 &0.000 &0.000 \\ 
0.000 &0.267 &0.000 &0.000 &0.000 \\ 
0.000 &0.000 &0.313 &0.000 &0.000 \\ 
0.000 &0.000 &0.000 &0.313 &0.000 \\ 
0.000 &0.000 &0.000 &0.000 &0.313 \\ 
\end{array}\right) $&$ \left( \begin{array}{ccccc}0.033 &-0.081 &0.000 &0.000 &0.000 \\ 
-0.081 &0.127 &0.000 &0.000 &0.000 \\ 
0.000 &0.000 &-0.016 &0.000 &0.000 \\ 
0.000 &0.000 &0.000 &0.148 &0.000 \\ 
0.000 &0.000 &0.000 &0.000 &0.148 \\ 
\end{array}\right) $\\ 
\hline  
LiOs & $ \left( \begin{array}{ccccc}0.386 &0.000 &0.000 &0.000 &0.000 \\ 
0.000 &0.386 &0.000 &0.000 &0.000 \\ 
0.000 &0.000 &0.243 &0.000 &0.000 \\ 
0.000 &0.000 &0.000 &0.243 &0.000 \\ 
0.000 &0.000 &0.000 &0.000 &0.243 \\ 
\end{array}\right) $&$ \left( \begin{array}{ccccc}0.047 &-0.117 &0.000 &0.000 &0.000 \\ 
-0.117 &0.182 &0.000 &0.000 &0.000 \\ 
0.000 &0.000 &-0.013 &0.000 &0.000 \\ 
0.000 &0.000 &0.000 &0.115 &0.000 \\ 
0.000 &0.000 &0.000 &0.000 &0.115 \\ 
\end{array}\right) $\\ 
\hline  
\end{tabular}  
}  
\end{table}  


==> Eccs_summary_Latex_5_onlytwo_Acoustic_B12 <==
\begin{table}  
\caption{\label{tab:ECCs_summary_all_onlytwoAcoustic_B12} 
$\Xi$ matrix for JT active centers in one convention unit cell. `All' and `Acoustic' distinguish the parameters from all phonons and the contribution from acoustic phonons, respectively. From the left to right, and from the top to bottom, the matrix elements correspond to JTD\_2, JTD\_3, JTD\_4, JTD\_5 and JTD\_6, respectively. The unit is $bohr^2/Ry$. `NaOs' and `LiOs' are for 'Ba$_2$NaOsO$_6$' and 'Ba$_2$LiOsO$_6$', respectively. } 
\resizebox{0.5\textwidth}{!}{  
\begin{tabular}{|c|c|c|}\hline  
&  All &  Acoustic  \\   
\hline  
& (0,0,0) (JTC1,JTC1) & (0,0,0) (JTC1,JTC1)  \\ \hline  
NaOs & $ \left( \begin{array}{ccccc}4.988 &0.000 &0.000 &0.000 &0.000 \\ 
0.000 &4.988 &0.000 &0.000 &0.000 \\ 
0.000 &0.000 &10.472 &0.000 &0.000 \\ 
0.000 &0.000 &0.000 &10.472 &0.000 \\ 
0.000 &0.000 &0.000 &0.000 &10.472 \\ 
\end{array}\right) $&$ \left( \begin{array}{ccccc}0.089 &-0.000 &0.000 &0.000 &0.000 \\ 
-0.000 &0.089 &-0.000 &-0.000 &0.000 \\ 
0.000 &-0.000 &0.030 &-0.000 &-0.000 \\ 
0.000 &-0.000 &-0.000 &0.030 &-0.000 \\ 
0.000 &0.000 &-0.000 &-0.000 &0.030 \\ 
\end{array}\right) $\\ 
\hline  
LiOs & $ \left( \begin{array}{ccccc}5.464 &0.000 &0.000 &0.000 &0.000 \\ 
0.000 &5.464 &0.000 &0.000 &0.000 \\ 
0.000 &0.000 &9.921 &0.000 &0.000 \\ 
0.000 &0.000 &0.000 &9.921 &0.000 \\ 
0.000 &0.000 &0.000 &0.000 &9.921 \\ 
\end{array}\right) $&$ \left( \begin{array}{ccccc}0.051 &-0.000 &-0.000 &0.000 &0.000 \\ 
-0.000 &0.051 &-0.000 &0.000 &-0.000 \\ 
-0.000 &-0.000 &0.051 &0.000 &0.000 \\ 
0.000 &0.000 &0.000 &0.051 &0.000 \\ 
0.000 &-0.000 &0.000 &0.000 &0.051 \\ 
\end{array}\right) $\\ 
\hline  
\end{tabular}  
}  
\end{table}  

